SkillsVote: Lifecycle Governance of Agent Skills from Collection, Recommendation to Evolution

Long-horizon LLM agents generate traces that could become reusable experience, but raw trajectories are noisy, local, and hard to govern. Agent Skills offer a structured artifact for combining procedural guidance, executable resources, and applicability boundaries. Yet open skill ecosystems contain redundant, uneven, environment-sensitive artifacts, and indiscriminate updates can pollute future context. We present SkillsVote, a lifecycle-governance framework for Agent Skills across collection, recommendation, attribution, and evolution. SkillsVote profiles a million-scale open source corpus for environment requirements, quality, and verifiability, and synthesizes tasks for verifiable skills. Before execution, it performs agentic library search over structured skill folders to expose instructional context. After execution, it decomposes trajectories into skill-linked subtasks, attributes outcomes to skill-guided execution, agent exploration, environment, and result signals, and admits only successful reusable discoveries to evidence-gated updates. Experiments on Terminal-Bench 2.0 and SWE-Bench Pro show that SkillsVote improves agent performance on challenging agentic coding benchmarks. The gains arise from two complementary pathways: online evolution over task streams at test time and offline transfer via frozen libraries built from either historical trajectories or curated open source skills.

==> assets/case_study/markdown-cache/45985999ff8ff02916dfb0813d904fec.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererSectionBegin
\markdownRendererSectionBegin
\markdownRendererHeadingTwo{Task Instruction}\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingThree{Lack of API Support for Managing Group Invitations Limits Extensibility}\markdownRendererInterblockSeparator
{}Group invitation logic for issuing, accepting, and rejecting invitations is handled through socket events and the web layer. The task requires authenticated HTTP API endpoints so external clients can issue, accept, and reject or rescind group invitations.\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererStrongEmphasis{Issue invite}: \markdownRendererCodeSpan{POST /groups/\markdownRendererLeftBrace{}slug\markdownRendererRightBrace{}/invites/\markdownRendererLeftBrace{}uid\markdownRendererRightBrace{}} lets a group owner or admin issue an invitation and log \markdownRendererCodeSpan{group-invite}.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{Accept invite}: \markdownRendererCodeSpan{PUT /groups/\markdownRendererLeftBrace{}slug\markdownRendererRightBrace{}/invites/\markdownRendererLeftBrace{}uid\markdownRendererRightBrace{}} lets the invited user accept their own invite. If \markdownRendererCodeSpan{uid} differs from the caller, return \markdownRendererCodeSpan{[[error:not-allowed]]}; if no invite exists, return \markdownRendererCodeSpan{[[error:not-invited]]}; log \markdownRendererCodeSpan{group-invite-accept}.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{Reject or rescind invite}: \markdownRendererCodeSpan{DELETE /groups/\markdownRendererLeftBrace{}slug\markdownRendererRightBrace{}/invites/\markdownRendererLeftBrace{}uid\markdownRendererRightBrace{}} lets the invited user reject or an owner/admin rescind an invite, with \markdownRendererCodeSpan{[[error:not-invited]]} or \markdownRendererCodeSpan{[[error:not-allowed]]} on invalid cases. Rejection by the invited user logs \markdownRendererCodeSpan{group-invite-reject}.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}The implementation should add exported functions \markdownRendererCodeSpan{issueInvite}, \markdownRendererCodeSpan{acceptInvite}, and \markdownRendererCodeSpan{rejectInvite} in \markdownRendererCodeSpan{src/api/groups.js}, add controllers in \markdownRendererCodeSpan{src/controllers/write/groups.js}, and update the web client and OpenAPI specification.\markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{Skill Recommendation}\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingThree{Recommended Skills}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererCodeSpan{nodebb-core-route-module}\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{nodebb-v3-write-api-repro}\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{nodebb-bootstrap-repro}\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{debug-http-status-api-errors}\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{nodebb-api-error-and-teaser-debug}\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{Usage Guide}\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{assets/case_study/markdown-cache/27a2cbd90f72198f6fb809f9f027465b.verbatim}{markdown}{markdown}\markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{Agent Trajectory Summary}\markdownRendererInterblockSeparator
{}<think>\markdownRendererParagraphSeparator
{}Scan the repository for group invitation logic, then add v3 write routes, controllers, API methods, client updates, OpenAPI entries, and an authenticated repro.\markdownRendererParagraphSeparator
{}</think>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}Inspect \markdownRendererCodeSpan{src/groups/invite.js}, \markdownRendererCodeSpan{src/api/groups.js}, \markdownRendererCodeSpan{src/controllers/write/groups.js}, and \markdownRendererCodeSpan{src/routes/write/groups.js}.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}Inspect the existing OpenAPI invite spec and group details client code.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}Create \markdownRendererCodeSpan{scripts/repro-group-invite-write-api.js} to exercise issue, accept, reject, and rescind flows through \markdownRendererCodeSpan{/api/v3/groups/:slug/invites/:uid}.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}Run the Mocha repro script.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}response>\markdownRendererParagraphSeparator
{}The first repro run fails because Redis is unavailable.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}response>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}Start Redis with \markdownRendererCodeSpan{redis-server --daemonize yes --port 6379} and confirm \markdownRendererCodeSpan{redis-cli -p 6379 ping} returns \markdownRendererCodeSpan{PONG}.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}response>\markdownRendererParagraphSeparator
{}The repro then reaches the application and confirms route absence before implementation.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}response>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}Patch the group API module, write controllers and routes, the web client, and the OpenAPI spec.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}Search for \markdownRendererCodeSpan{formatApiResponse} and existing \markdownRendererCodeSpan{[[error:not-allowed]]} handling to align response envelopes and statuses.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}Patch status mapping and serializer behavior, then rerun the repro.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}<answer>\markdownRendererParagraphSeparator
{}The local repro passes for the new group invite Write API, but the verifier still reports six private failures.\markdownRendererParagraphSeparator
{}</answer>\markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{Distilled Subtasks}\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingThree{Subtask 1}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererStrongEmphasis{goal}: Locate the existing group invitation implementation and identify where to add equivalent authenticated HTTP endpoints.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{summary}: The agent found group invite logic in the socket and group-invite modules, then mapped the v3 write route, controller, and API modules that needed to be extended. It confirmed invite HTTP routes were missing or commented out and that OpenAPI only documented \markdownRendererCodeSpan{GET /groups/\markdownRendererLeftBrace{}slug\markdownRendererRightBrace{}/invites}.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{attribution}: \markdownRendererCodeSpan{success\markdownRendererUnderscore{}no\markdownRendererUnderscore{}skill\markdownRendererUnderscore{}seen}\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{Subtask 2}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererStrongEmphasis{goal}: Create an executable end-to-end repro that boots NodeBB with the test database mock and exercises the new invite HTTP routes.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{summary}: The agent created \markdownRendererCodeSpan{scripts/repro-group-invite-write-api.js}, booted through \markdownRendererCodeSpan{test/mocks/databasemock}, created users and a private group, logged in to obtain authenticated jars, and issued HTTP \markdownRendererCodeSpan{POST}, \markdownRendererCodeSpan{PUT}, and \markdownRendererCodeSpan{DELETE} requests against \markdownRendererCodeSpan{/api/v3/groups/:slug/invites/:uid}. The initial run failed with Redis \markdownRendererCodeSpan{ECONNREFUSED}; after starting Redis, the repro confirmed the pre-implementation 404.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{exploration}: For NodeBB end-to-end repros, use a Mocha script requiring \markdownRendererCodeSpan{test/mocks/databasemock}, use \markdownRendererCodeSpan{test/helpers} for login and CSRF handling, then exercise HTTP routes; if bootstrap fails with Redis \markdownRendererCodeSpan{ECONNREFUSED}, start local Redis on that host and port before rerunning.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{attribution}: \markdownRendererCodeSpan{success\markdownRendererUnderscore{}skill\markdownRendererUnderscore{}used\markdownRendererUnderscore{}with\markdownRendererUnderscore{}extra\markdownRendererUnderscore{}exploration}\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{skill\markdownRendererUnderscore{}refs}: \markdownRendererCodeSpan{nodebb-bootstrap-repro} Mocha, databasemock, and authenticated HTTP pattern.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingFour{\markdownRendererCodeSpan{SKILL.md}}\markdownRendererInterblockSeparator
{}Line 24-42\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{assets/case_study/markdown-cache/42014b448519917ebb6e2156f2c263c8.verbatim}{markdown}{markdown}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{Subtask 3}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererStrongEmphasis{goal}: Implement authenticated v3 write API endpoints to issue, accept, and reject or rescind group invitations using \markdownRendererCodeSpan{slug} and \markdownRendererCodeSpan{uid} path parameters.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{summary}: The agent implemented \markdownRendererCodeSpan{groupsAPI.issueInvite}, \markdownRendererCodeSpan{groupsAPI.acceptInvite}, and \markdownRendererCodeSpan{groupsAPI.rejectInvite} in \markdownRendererCodeSpan{src/api/groups.js} with permission checks and event logging, then added controllers and routes for \markdownRendererCodeSpan{POST}, \markdownRendererCodeSpan{PUT}, and \markdownRendererCodeSpan{DELETE} at \markdownRendererCodeSpan{/api/v3/groups/:slug/invites/:uid}.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{attribution}: \markdownRendererCodeSpan{success\markdownRendererUnderscore{}no\markdownRendererUnderscore{}skill\markdownRendererUnderscore{}seen}\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{Subtask 4}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererStrongEmphasis{goal}: Update the web client and OpenAPI write specification to reflect and use the new invite management routes.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{summary}: The agent updated the group-details client to use the v3 API module for invite issue, accept, reject, and rescind actions, and added OpenAPI path/spec files for \markdownRendererCodeSpan{POST}, \markdownRendererCodeSpan{PUT}, and \markdownRendererCodeSpan{DELETE} on \markdownRendererCodeSpan{/groups/\markdownRendererLeftBrace{}slug\markdownRendererRightBrace{}/invites/\markdownRendererLeftBrace{}uid\markdownRendererRightBrace{}}.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{attribution}: \markdownRendererCodeSpan{uncertain\markdownRendererUnderscore{}no\markdownRendererUnderscore{}judge}\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{Subtask 5}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererStrongEmphasis{goal}: Ensure invite endpoint errors return correct HTTP statuses and preserve canonical error keys in API responses.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{summary}: The agent observed a repro failure where \markdownRendererCodeSpan{[[error:not-allowed]]} surfaced with HTTP \markdownRendererCodeSpan{400} and a translated \markdownRendererCodeSpan{not-allowed} message. It adjusted \markdownRendererCodeSpan{src/controllers/helpers.js} to map \markdownRendererCodeSpan{[[error:not-allowed]]} and \markdownRendererCodeSpan{[[error:not-invited]]} to HTTP \markdownRendererCodeSpan{403} and preserve untranslated keys for \markdownRendererCodeSpan{/api/v3}; the repro then passed.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{exploration}: When write API tests require exact error keys, avoid automatic translation in the \markdownRendererCodeSpan{/api/v3} serializer and map common permission-related keys to \markdownRendererCodeSpan{403}; otherwise callers may see translated strings and inconsistent status codes.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{attribution}: \markdownRendererCodeSpan{success\markdownRendererUnderscore{}no\markdownRendererUnderscore{}skill\markdownRendererUnderscore{}seen}\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{Subtask 6}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererStrongEmphasis{goal}: Achieve full private test suite compliance for the implemented invite API changes without regressing unrelated API behavior.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{summary}: The local repro passed, but the verifier reported \markdownRendererCodeSpan{421/427} private tests passing with six failures remaining, suggesting incomplete edge-case handling or regressions around global API status/translation behavior or permission semantics.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{attribution}: \markdownRendererCodeSpan{fail\markdownRendererUnderscore{}agent\markdownRendererUnderscore{}limit}\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{Skill Evolution}\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingThree{[edit] nodebb-bootstrap-repro}\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingFour{\markdownRendererCodeSpan{SKILL.md}}\markdownRendererInterblockSeparator
{}Line 22-29\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{assets/case_study/markdown-cache/b32cc3b32e1b35e16225ba927806b3c6.verbatim}{markdown}{markdown}\markdownRendererInterblockSeparator
{}Line 65-68\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{assets/case_study/markdown-cache/1db09c76426cf5a04f5eae2e3974925f.verbatim}{markdown}{markdown}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd 
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererDocumentEnd

==> assets/case_study/markdown-cache/6b1a2b053c0e34a94d7f11ce9e4b0b07.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererSectionBegin
\markdownRendererSectionBegin
\markdownRendererHeadingTwo{Task Instruction}\markdownRendererInterblockSeparator
{}Configure an Apache web server environment to serve content with comprehensive logging and rate limiting.\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererStrongEmphasis{Apache2}: installed and available via \markdownRendererCodeSpan{apache2ctl}.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{Port}: listen on port \markdownRendererCodeSpan{9090}.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{Document Root}: serve static content from \markdownRendererCodeSpan{/srv/www/content}.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{Log Format}: include timestamps, HTTP methods, status codes, response sizes, and referrers.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}The task requires a \markdownRendererCodeSpan{*:9090} virtual host with \markdownRendererCodeSpan{ServerName localhost}, detailed access and error logs under \markdownRendererCodeSpan{/var/log/apache2}, a maximum of 20 concurrent connections per IP, a custom \markdownRendererCodeSpan{/403.html} page, required Apache modules, site activation, server startup, and runtime verification.\markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{Agent Trajectory Summary}\markdownRendererInterblockSeparator
{}<think>\markdownRendererParagraphSeparator
{}Inspect the existing Apache layout and repository-specific configuration so the changes can be made persistently.\markdownRendererParagraphSeparator
{}</think>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}Run \markdownRendererCodeSpan{apache2ctl -v}, list loaded modules, and search files under \markdownRendererCodeSpan{/etc/apache2}.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}Read the benchmark site configuration and \markdownRendererCodeSpan{/etc/apache2/ports.conf}.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}Search Apache packages for connection-limiting modules such as \markdownRendererCodeSpan{qos}, \markdownRendererCodeSpan{evasive}, and \markdownRendererCodeSpan{ratelimit}.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}Install \markdownRendererCodeSpan{libapache2-mod-qos} and inspect \markdownRendererCodeSpan{QS\markdownRendererUnderscore{}} directives.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}Validate the Apache configuration with \markdownRendererCodeSpan{apache2ctl -t} and inspect vhost bindings with \markdownRendererCodeSpan{apache2ctl -S}.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}response>\markdownRendererParagraphSeparator
{}Live requests to \markdownRendererCodeSpan{http://127.0.0.1:9090/} and \markdownRendererCodeSpan{/403.html} verify serving and custom error behavior.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}response>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}response>\markdownRendererParagraphSeparator
{}A denied real path under the document root produces the expected access and error log entries.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}response>\markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{Distilled Subtasks}\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingThree{Subtask 1}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererStrongEmphasis{goal}: Inspect the Apache environment and locate the existing benchmark site configuration.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{exploration}: On Ubuntu Apache layouts, persistent port bindings belong in \markdownRendererCodeSpan{ports.conf}, while site-specific behavior should live in \markdownRendererCodeSpan{sites-available} and be activated via symlinks. Existing benchmark site configs can often be adapted rather than recreated.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{attribution}: \markdownRendererCodeSpan{success\markdownRendererUnderscore{}no\markdownRendererUnderscore{}skill\markdownRendererUnderscore{}seen}\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{Subtask 2}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererStrongEmphasis{goal}: Implement persistent Apache configuration for port \markdownRendererCodeSpan{9090}, custom logging, and per-IP connection limiting.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{exploration}: For Apache concurrency limits, \markdownRendererCodeSpan{mod\markdownRendererUnderscore{}qos} provides \markdownRendererCodeSpan{QS\markdownRendererUnderscore{}SrvMaxConnPerIP}, which is practical when the stock module set only includes \markdownRendererCodeSpan{mod\markdownRendererUnderscore{}ratelimit} for bandwidth throttling rather than true connection concurrency control.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{attribution}: \markdownRendererCodeSpan{success\markdownRendererUnderscore{}no\markdownRendererUnderscore{}skill\markdownRendererUnderscore{}seen}\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{Subtask 3}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererStrongEmphasis{goal}: Start Apache and verify the server responds correctly on port \markdownRendererCodeSpan{9090} with the expected logging and 403 behavior.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{exploration}: A reliable Apache 403 test is easier to validate by denying a real directory under the document root than by relying on a nonexistent path or rewrite rule.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{attribution}: \markdownRendererCodeSpan{success\markdownRendererUnderscore{}no\markdownRendererUnderscore{}skill\markdownRendererUnderscore{}seen}\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{Skill Evolution}\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingThree{[create] ubuntu-apache-vhost}\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{assets/case_study/markdown-cache/e3a48a7d642e6f811a47fad1ff3a8163.verbatim}{markdown}{markdown}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererDocumentEnd

==> assets/case_study/markdown-cache/b8bf49084dcafacfa5ca0f93d3a44a81.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererSectionBegin
\markdownRendererSectionBegin
\markdownRendererHeadingTwo{Task Instruction}\markdownRendererInterblockSeparator
{}Configure a Git server so that a user can run:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererCodeSpan{git clone user@server:/git/server}\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{echo "hello world" > hello.html}\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{git add hello.html}\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{git commit -m "add hello.html"}\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{git push origin master}\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}The pushed data should be served by a webserver on port \markdownRendererCodeSpan{8080}; \markdownRendererCodeSpan{curl http://server:8080/hello.html} should return \markdownRendererCodeSpan{hello world}. Login setup is assumed to be handled externally.\markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{Agent Trajectory Summary}\markdownRendererInterblockSeparator
{}<think>\markdownRendererParagraphSeparator
{}Inspect the workspace and wire a Git receive/update flow to an HTTP serving path so pushed files materialize on port \markdownRendererCodeSpan{8080}.\markdownRendererParagraphSeparator
{}</think>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}Probe available runtimes and service binaries, including Python, Node.js, Ruby, Go, \markdownRendererCodeSpan{sshd}, and \markdownRendererCodeSpan{git}.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}<think>\markdownRendererParagraphSeparator
{}Use a bare repository with a \markdownRendererCodeSpan{post-receive} hook that checks out the pushed branch into a web root, plus a small static server on \markdownRendererCodeSpan{8080}.\markdownRendererParagraphSeparator
{}</think>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}Attempt to install Git with \markdownRendererCodeSpan{apt-get update} and \markdownRendererCodeSpan{apt-get install -y git}.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}response>\markdownRendererParagraphSeparator
{}\markdownRendererCodeSpan{apt-get} cannot proceed because \markdownRendererCodeSpan{/var/lib/apt/lists/lock} is held by another process.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}response>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}Kill stuck \markdownRendererCodeSpan{apt-get} processes and continue with generated setup files.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}<answer>\markdownRendererParagraphSeparator
{}The agent writes setup scripts and documentation, but cannot fully exercise the Git hook because Git installation failed in the environment.\markdownRendererParagraphSeparator
{}</answer>
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererDocumentEnd

==> assets/case_study/markdown-cache/cd5fe74581e6f830f7f97045b4acb425.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererSectionBegin
\markdownRendererSectionBegin
\markdownRendererHeadingTwo{Task Instruction}\markdownRendererInterblockSeparator
{}Configure Apache2 to implement custom port listening and advanced access log recording.\markdownRendererInterblockSeparator
{}\markdownRendererOlBeginTight
\markdownRendererOlItemWithNumber{1}Create \markdownRendererCodeSpan{analytics-site.conf} under \markdownRendererCodeSpan{/etc/apache2/sites-available/}, using \markdownRendererCodeSpan{<VirtualHost *:9090>}, \markdownRendererCodeSpan{ServerName localhost}, and \markdownRendererCodeSpan{DocumentRoot /var/www/content}.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{2}Configure \markdownRendererCodeSpan{/var/log/apache2/traffic-access.log} with the format \markdownRendererCodeSpan{\markdownRendererPercentSign{}t \markdownRendererPercentSign{}m \markdownRendererPercentSign{}s \markdownRendererPercentSign{}\markdownRendererLeftBrace{}Referer\markdownRendererRightBrace{}i [\markdownRendererPercentSign{}a]}.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{3}Configure \markdownRendererCodeSpan{/var/www/content} with \markdownRendererCodeSpan{Options Indexes FollowSymLinks}, \markdownRendererCodeSpan{AllowOverride None}, and \markdownRendererCodeSpan{Require all granted}.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{4}Add \markdownRendererCodeSpan{Listen 9090} at the end of the configuration file.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{5}Enable the site with \markdownRendererCodeSpan{a2ensite analytics-site.conf}.\markdownRendererOlItemEnd 
\markdownRendererOlEndTight \markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{Skill Recommendation}\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingThree{Recommended Skills}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererCodeSpan{ubuntu-apache-vhost}\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{Usage Guide}\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{assets/case_study/markdown-cache/110251a27bf8842991f2fe1373f6d026.verbatim}{markdown}{markdown}\markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{Agent Trajectory Summary}\markdownRendererInterblockSeparator
{}<think>\markdownRendererParagraphSeparator
{}Use \markdownRendererCodeSpan{ubuntu-apache-vhost} because the task is an Apache vhost and listener configuration task; inspect the current layout before editing.\markdownRendererParagraphSeparator
{}</think>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}Read the \markdownRendererCodeSpan{ubuntu-apache-vhost} skill file.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}List Apache configuration files and inspect current bindings with \markdownRendererCodeSpan{apache2ctl -S}.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}Check service state using \markdownRendererCodeSpan{systemctl is-active apache2} or \markdownRendererCodeSpan{service apache2 status}.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}Enable \markdownRendererCodeSpan{analytics-site.conf}, validate syntax with \markdownRendererCodeSpan{apache2ctl -t}, and start Apache with \markdownRendererCodeSpan{service apache2 start}.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}response>\markdownRendererParagraphSeparator
{}Requests to \markdownRendererCodeSpan{http://localhost:9090/} with a referrer create the expected \markdownRendererCodeSpan{/var/log/apache2/traffic-access.log} entries.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}response>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}Confirm the listener with \markdownRendererCodeSpan{ss -ltnp} and inspect the site file for \markdownRendererCodeSpan{traffic-access} and \markdownRendererCodeSpan{Listen 9090}.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}call>\markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{Distilled Subtasks}\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingThree{Subtask 1}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererStrongEmphasis{goal}: Inspect the Apache environment and determine the correct configuration path for a \markdownRendererCodeSpan{9090} analytics vhost.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{exploration}: Use \markdownRendererCodeSpan{apache2ctl -S} together with the Debian/Ubuntu Apache directory layout to verify existing listeners and vhost bindings before making changes.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{attribution}: \markdownRendererCodeSpan{success\markdownRendererUnderscore{}skill\markdownRendererUnderscore{}used\markdownRendererUnderscore{}with\markdownRendererUnderscore{}extra\markdownRendererUnderscore{}exploration}\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{skill\markdownRendererUnderscore{}linked}: \markdownRendererCodeSpan{ubuntu-apache-vhost}\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{skill\markdownRendererUnderscore{}refs}: \markdownRendererCodeSpan{SKILL.md} line 14-18.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingFour{\markdownRendererCodeSpan{SKILL.md}}\markdownRendererInterblockSeparator
{}Line 14-18\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{assets/case_study/markdown-cache/2c8eb7276e8c4ffed492eee765185cab.verbatim}{markdown}{markdown}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{Subtask 2}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererStrongEmphasis{goal}: Implement and activate the analytics Apache site on port \markdownRendererCodeSpan{9090} with the required document root, log format, and homepage.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{exploration}: Placing \markdownRendererCodeSpan{Listen 9090} at the end of the site file worked in this environment, and \markdownRendererCodeSpan{service apache2 start} was the viable startup path when \markdownRendererCodeSpan{systemctl} was unavailable.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{attribution}: \markdownRendererCodeSpan{success\markdownRendererUnderscore{}skill\markdownRendererUnderscore{}used\markdownRendererUnderscore{}with\markdownRendererUnderscore{}extra\markdownRendererUnderscore{}exploration}\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{skill\markdownRendererUnderscore{}linked}: \markdownRendererCodeSpan{ubuntu-apache-vhost}\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{skill\markdownRendererUnderscore{}refs}: \markdownRendererCodeSpan{SKILL.md} line 24-26.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingFour{\markdownRendererCodeSpan{SKILL.md}}\markdownRendererInterblockSeparator
{}Line 24-26\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{assets/case_study/markdown-cache/6d1748f0bf945187b52b12b8c3de2410.verbatim}{markdown}{markdown}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{Subtask 3}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererStrongEmphasis{goal}: Verify the deployed Apache site, response body, and custom access-log behavior against the benchmark expectations.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{exploration}: Full validation required both runtime probing and file inspection because the verifier checks HTTP response, log creation, exact log formatting, enabled-site state, and static config content.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{attribution}: \markdownRendererCodeSpan{success\markdownRendererUnderscore{}no\markdownRendererUnderscore{}skill\markdownRendererUnderscore{}seen}\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{Skill Evolution}\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingThree{[edit] ubuntu-apache-vhost}\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingFour{\markdownRendererCodeSpan{SKILL.md}}\markdownRendererInterblockSeparator
{}Line 14-20\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{assets/case_study/markdown-cache/a0efe2c7f033f9419966e383c9a8c9fc.verbatim}{markdown}{markdown}\markdownRendererInterblockSeparator
{}Line 40\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{assets/case_study/markdown-cache/11c8b6345ee68670dcc0004c2e9ff6d6.verbatim}{markdown}{markdown}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd 
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererDocumentEnd

==> assets/case_study/markdown-cache/f689cf36309a7dbb9bd065f3cbde3a46.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererSectionBegin
\markdownRendererSectionBegin
\markdownRendererHeadingTwo{Task Instruction}\markdownRendererInterblockSeparator
{}Configure a Git server so that a user can run:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererCodeSpan{git clone user@server:/git/server}\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{echo "hello world" > hello.html}\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{git add hello.html}\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{git commit -m "add hello.html"}\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{git push origin master}\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}The pushed data should be served by a webserver on port \markdownRendererCodeSpan{8080}; \markdownRendererCodeSpan{curl http://server:8080/hello.html} should return \markdownRendererCodeSpan{hello world}. Login setup is assumed to be handled externally.\markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{Skill Recommendation}\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingThree{Recommended Skills}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererCodeSpan{ubuntu-apache-vhost}\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{Usage Guide}\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{assets/case_study/markdown-cache/76a20c6be6b5972f9893d7558b1f8362.verbatim}{markdown}{markdown}\markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{Agent Trajectory Summary}\markdownRendererInterblockSeparator
{}<think>\markdownRendererParagraphSeparator
{}Use \markdownRendererCodeSpan{ubuntu-apache-vhost} for the HTTP side, inspect the Apache layout, and then wire the bare Git repository plus deployment hook so pushes land in Apache's document root.\markdownRendererParagraphSeparator
{}</think>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}Read the \markdownRendererCodeSpan{ubuntu-apache-vhost} skill file.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}Run \markdownRendererCodeSpan{apache2ctl -S} and check Apache service state with \markdownRendererCodeSpan{service apache2 status} or \markdownRendererCodeSpan{systemctl status apache2}.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}Install the required packages: Apache, Git, and OpenSSH server.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}Inspect \markdownRendererCodeSpan{/etc/apache2/ports.conf} and existing site configurations.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}Create the bare repository, add an executable \markdownRendererCodeSpan{post-receive} hook, enable the Apache site, and run \markdownRendererCodeSpan{apache2ctl -t}.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}call>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}response>\markdownRendererParagraphSeparator
{}\markdownRendererCodeSpan{apache2ctl -S} reports a \markdownRendererCodeSpan{*:8080} vhost from \markdownRendererCodeSpan{/etc/apache2/sites-enabled/git-server.conf}.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}response>\markdownRendererParagraphSeparator
{}<tool\markdownRendererUnderscore{}response>\markdownRendererParagraphSeparator
{}A local commit and push to \markdownRendererCodeSpan{/git/server}, followed by \markdownRendererCodeSpan{curl http://127.0.0.1:8080/hello.html}, returns \markdownRendererCodeSpan{hello world}.\markdownRendererParagraphSeparator
{}</tool\markdownRendererUnderscore{}response>\markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{Distilled Subtasks}\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingThree{Subtask 1}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererStrongEmphasis{goal}: Configure Apache to serve a persistent virtual host on port \markdownRendererCodeSpan{8080} from a stable document root.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{summary}: The agent installed packages, configured \markdownRendererCodeSpan{/etc/apache2/ports.conf}, added a \markdownRendererCodeSpan{*:8080} vhost with \markdownRendererCodeSpan{DocumentRoot /srv/git-server/www}, enabled the site, and verified it with \markdownRendererCodeSpan{apache2ctl -t}, \markdownRendererCodeSpan{apache2ctl -S}, and \markdownRendererCodeSpan{curl}.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{exploration}: On Ubuntu/Debian, persistent Apache port binding should be placed in \markdownRendererCodeSpan{ports.conf}; site config should live in \markdownRendererCodeSpan{sites-available}; \markdownRendererCodeSpan{apache2ctl -S} plus a live HTTP request are fast checks that the vhost is bound and serving from the intended document root.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{attribution}: \markdownRendererCodeSpan{success\markdownRendererUnderscore{}skill\markdownRendererUnderscore{}used\markdownRendererUnderscore{}with\markdownRendererUnderscore{}extra\markdownRendererUnderscore{}exploration}\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{skill\markdownRendererUnderscore{}linked}: \markdownRendererCodeSpan{ubuntu-apache-vhost}\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{skill\markdownRendererUnderscore{}refs}: \markdownRendererCodeSpan{SKILL.md} line 14-20, line 24-26, and line 36-40.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingFour{\markdownRendererCodeSpan{SKILL.md}}\markdownRendererInterblockSeparator
{}Line 14-20\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{assets/case_study/markdown-cache/a0efe2c7f033f9419966e383c9a8c9fc.verbatim}{markdown}{markdown}\markdownRendererInterblockSeparator
{}Line 24-26\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{assets/case_study/markdown-cache/62063063940eb29caa172d8d6841b851.verbatim}{markdown}{markdown}\markdownRendererInterblockSeparator
{}Line 36-40\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{assets/case_study/markdown-cache/a6d3bffe3fc654efda54bb26edcb144b.verbatim}{markdown}{markdown}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{Subtask 2}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererStrongEmphasis{goal}: Create a bare Git repository with a deploy hook that publishes pushed \markdownRendererCodeSpan{master} contents into the Apache document root.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{summary}: The agent created \markdownRendererCodeSpan{/git/server} as a bare repository and \markdownRendererCodeSpan{/srv/git-server/www} as the deployment target, added an executable \markdownRendererCodeSpan{post-receive} hook, pushed \markdownRendererCodeSpan{hello.html}, and verified that \markdownRendererCodeSpan{curl} returned \markdownRendererCodeSpan{hello world}.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{exploration}: A bare repository can serve as a lightweight deployment endpoint when \markdownRendererCodeSpan{post-receive} checks out the pushed branch into the web root and cleans stray files so the web root mirrors the branch.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{attribution}: \markdownRendererCodeSpan{success\markdownRendererUnderscore{}no\markdownRendererUnderscore{}skill\markdownRendererUnderscore{}seen}\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{Skill Evolution}\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingThree{[edit] ubuntu-apache-vhost}\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingFour{\markdownRendererCodeSpan{SKILL.md}}\markdownRendererInterblockSeparator
{}Line 40\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{assets/case_study/markdown-cache/bb71a627adf43100deebb6d788975a23.verbatim}{markdown}{markdown}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{[create] git-web-publish}\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{assets/case_study/markdown-cache/8ba52c3287c854019a0b32642129cf43.verbatim}{markdown}{markdown}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererDocumentEnd

==> assets/case_study/markdown-cache/frozenCache.tex <==
\expandafter\global\expandafter\def\csname markdownFrozenCache0\endcsname{\input{assets/case_study/markdown-cache/6b1a2b053c0e34a94d7f11ce9e4b0b07.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache1\endcsname{\input{assets/case_study/markdown-cache/cd5fe74581e6f830f7f97045b4acb425.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache2\endcsname{\input{assets/case_study/markdown-cache/f689cf36309a7dbb9bd065f3cbde3a46.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache3\endcsname{\input{assets/case_study/markdown-cache/b8bf49084dcafacfa5ca0f93d3a44a81.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache4\endcsname{\input{assets/case_study/markdown-cache/45985999ff8ff02916dfb0813d904fec.md.tex}\relax}

